AssetHarvester: A Static Analysis Tool for Detecting Secret-Asset Pairs in Software Artifacts

GitGuardian monitored secrets exposure in public GitHub repositories and reported that developers leaked over 12 million secrets (database and other credentials) in 2023, indicating a 113% surge from 2021. Despite the availability of secret detection tools, developers ignore the tools' reported warnings because of false positives (25%-99%). However, each secret protects assets of different values accessible through asset identifiers (a DNS name and a public or private IP address). The asset information for a secret can aid developers in filtering false positives and prioritizing secret removal from the source code. However, existing secret detection tools do not provide the asset information, thus presenting difficulty to developers in filtering secrets only by looking at the secret value or finding the assets manually for each reported secret. The goal of our study is to aid software practitioners in prioritizing secrets removal by providing the assets information protected by the secrets through our novel static analysis tool. We present AssetHarvester, a static analysis tool to detect secret-asset pairs in a repository. Since the location of the asset can be distant from where the secret is defined, we investigated secret-asset co-location patterns and found four patterns. To identify the secret-asset pairs of the four patterns, we utilized three approaches (pattern matching, data flow analysis, and fast-approximation heuristics). We curated a benchmark of 1,791 secret-asset pairs of four database types extracted from 188 public GitHub repositories to evaluate the performance of AssetHarvester. AssetHarvester demonstrates precision of (97%), recall (90%), and F1-score (94%) in detecting secret-asset pairs. Our findings indicate that data flow analysis employed in AssetHarvester detects secret-asset pairs with 0% false positives and aids in improving recall of secret detection tools.

==> Sections/DataStorage.tex <==
Our dataset, AssetBench, is stored in Google BigQuery (Dataset ID: \textit{dev-range-351901.assetbench.assets}) as a relational structured data. The dataset can be accessed and expanded by users through SQL queries. However, due to the sensitive nature of the dataset, we will provide access to the dataset to only selected researchers and tool developers. Those who require access need to contact us through email.




==> Sections/Test.tex <==
% \textbf{AssetHarvester can be extended to detect non-database assets for corresponding secrets.} In our study, we detected assets of the corresponding secrets of four databases. However, the found secret-asset co-location patterns (Section~\ref{AssetPatterns}) also apply to non-database secret-asset pairs. For example, as shown in Pattern 1, secret and asset can be present in the same line and string. Similar to a database connection string, an API URL can contain both the secret and asset such as \texttt{\seqsplit{"https://api.openweathermap.org/weather?apikey=xxxxxxxx"}} where API key is the secret and URL is the asset. Since each vendor follows a specific format for API URLs, regex can be formulated for the API URLs and added to the regex list of AssetHarvester (Section~\ref{PatternMatching}). In addition, new sinks for non-database secret-asset pairs can be identified and added to the existing sinks for data flow analysis (Section~\ref{DataFlowAnalysis}). For example, the \texttt{get}, \texttt{post}, or \texttt{put} methods of \texttt{request} package~\cite{requestpackage} in Python act as sinks to API URLs.


AssetHarvester can be extended to detect non-database assets for corresponding secrets. In our study, we detected assets of the corresponding secrets of four databases. However, the found secret-asset co-location patterns (Section~\ref{AssetPatterns}) also apply to other databases and non-database secret-asset pairs. We observed a random sample of 10 secrets for each secret type from SecretBench and identified the asset types protected by the secrets into four categories. Below, we provide the asset categories and discuss how AssetHarvester can be extended to each asset category. 

\textit{Database Servers} Except the four databases studied in this work, AssetHarvester can be extended to identify other databases such as Oracle and MariaDB. Since, these databases also have a specific connection string format containing the secret and asset values, we can formulate regex to identify the secret-asset pair. For example, an Oracle connection string is \texttt{\seqsplit{"User Id=scott;password=tiger;data source=10.0.0.1"}}. In addition, we can add the driver functions of these databases as new sinks for secret and asset values. For example, \texttt{cx\_Oracle} is a Python database driver for connecting to Oracle database. 

==> Tables/BaseLineComparisonCopy.tex <==
\begin{table}[]
\begin{center}
\caption{Comparison of AssetHarvester with 9 Baseline Secret Detection Tools on Secret Detection}
\label{baseline-comparison}
\small
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Tool} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Precision \\ (TP, FP)\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Recall \\ (TP, FN)\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}F1\end{tabular}}} \\ \hline \hline
git-secrets  & 0.04 (1460,65)  & 0.01 (31,2083) & 0.02 \\ \hline
Gitleaks      & 0.21 (220,45)  & 0.02 (37,2077)   & 0.04 \\ \hline
Repo-supervisor    &  0.31 (1270,391)  & 0.17 (364,1750)   & 0.22 \\ \hline
TruffleHog & 0.19 (5666,1068)     & 0.40 (851,1263)     & 0.26 \\ \hline
Whispers & 0.06 (2203,147)     & 0.05 (112,2002)    & 0.05 \\ \hline
Commercial X & 0.35 (7260,2511)    & 0.28 (589,1525)    & 0.31 \\ \hline
ggshield & 0.49 (1972,969)    & 0.16 (330,1784)    & 0.24 \\ \hline
GitHub-scanner & 0.00 (0,0)    & 0.00 (0,0)    & 0.00 \\ \hline
Spectralops & 0.15 (574,88)    & 0.29 (609,1505)    & 0.20 \\ \hline
\cellcolor[HTML]{C0C0C0}AssetHarvester    & \cellcolor[HTML]{C0C0C0}0.92 (2298,89) & \cellcolor[HTML]{C0C0C0}0.90 (1892,222) & \cellcolor[HTML]{C0C0C0}0.90 \\ \hline
\end{tabular}
\end{center}
\end{table}

==> Tables/SameSecretAsset.tex <==
\begin{table*}[ht!]
\begin{center}
\caption{Statistics of the count of different asset values protected by five common secrets in AssetBench}
\label{same-secret-asset-values}
\small
\begin{tabular}{|l|l|lllll|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Asset Type}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Asset Example}}} &
  \multicolumn{5}{c|}{\textbf{Common Secrets}} \\ \cline{3-7} 
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{l|}{\textbf{123456}} &
  \multicolumn{1}{l|}{\textbf{root}} &
  \multicolumn{1}{l|}{\textbf{admin}} &
  \multicolumn{1}{l|}{\textbf{test}} &
  \textbf{pwd123} \\ \hline
\textbf{Localhost}           & localhost, 127.0.0.1          & \multicolumn{1}{l|}{33} & \multicolumn{1}{l|}{25} & \multicolumn{1}{l|}{9} & \multicolumn{1}{l|}{13} & 4 \\ \hline
\textbf{Template DNS}        & your-project-id.instance-name & \multicolumn{1}{l|}{0}  & \multicolumn{1}{l|}{8}  & \multicolumn{1}{l|}{0} & \multicolumn{1}{l|}{2}  & 0 \\ \hline
\textbf{DNS}                 & ds053958.mongolab.com         & \multicolumn{1}{l|}{11} & \multicolumn{1}{l|}{11} & \multicolumn{1}{l|}{1} & \multicolumn{1}{l|}{4}  & 3 \\ \hline
\textbf{Template IP Address} & ip:port                       & \multicolumn{1}{l|}{0}  & \multicolumn{1}{l|}{0}  & \multicolumn{1}{l|}{0} & \multicolumn{1}{l|}{1}  & 1 \\ \hline
\textbf{Private IP Address}  & 192.168.1.116, 10.0.0.1                 & \multicolumn{1}{l|}{3}  & \multicolumn{1}{l|}{19} & \multicolumn{1}{l|}{6} & \multicolumn{1}{l|}{6}  & 1 \\ \hline
\textbf{Public IP Address}   & 111.230.140.27                & \multicolumn{1}{l|}{4}  & \multicolumn{1}{l|}{9}  & \multicolumn{1}{l|}{0} & \multicolumn{1}{l|}{0}  & 0 \\ \hline
\textbf{Reserved IP Address} & 0.0.0.0                       & \multicolumn{1}{l|}{0}  & \multicolumn{1}{l|}{1}  & \multicolumn{1}{l|}{0} & \multicolumn{1}{l|}{0}  & 1 \\ \hline
\end{tabular}
\end{center}
\end{table*}
